K-independent percolation on trees

Consider the class of k-independent bond, respectively site, percolations with parameter p on an infinite tree T. We derive tight bounds on p for both a.s. percolation and a.s. nonpercolation. The bounds are continuous functions of k and the branching number of T. This extends previous results by Lyons for the independent case (k=0) and by Bollob\`as & Balister for 1-independent bond percolations. Central to our argumentation are moment method bounds \`a la Lyons supplemented by explicit percolation models \`a la Bollob\`as & Balister. An indispensable tool is the minimality and explicit construction of Shearer's measure on the k-fuzz of Z.

==> COMMON/latex/macro_general.tex <==
% general helpers
\newcommand{\Comment}[1]{}
\newcommand{\Undefine}[1]{
	\makeatletter
	\let#1\@undefined
}
\usepackage{color}
\newcommand{\Highlight}[1]{\textcolor{magenta}{\mathbf{#1}}}


